Language in a Bottle: Language Model Guided Concept Bottlenecks for Interpretable Image Classification

Concept Bottleneck Models (CBM) are inherently interpretable models that factor model decisions into human-readable concepts. They allow people to easily understand why a model is failing, a critical feature for high-stakes applications. CBMs require manually specified concepts and often under-perform their black box counterparts, preventing their broad adoption. We address these shortcomings and are first to show how to construct high-performance CBMs without manual specification of similar accuracy to black box models. Our approach, Language Guided Bottlenecks (LaBo), leverages a language model, GPT-3, to define a large space of possible bottlenecks. Given a problem domain, LaBo uses GPT-3 to produce factual sentences about categories to form candidate concepts. LaBo efficiently searches possible bottlenecks through a novel submodular utility that promotes the selection of discriminative and diverse information. Ultimately, GPT-3's sentential concepts can be aligned to images using CLIP, to form a bottleneck layer. Experiments demonstrate that LaBo is a highly effective prior for concepts important to visual recognition. In the evaluation with 11 diverse datasets, LaBo bottlenecks excel at few-shot classification: they are 11.7% more accurate than black box linear probes at 1 shot and comparable with more data. Overall, LaBo demonstrates that inherently interpretable models can be widely applied at similar, or better, performance than black box approaches.

==> tables/add_visual.tex <==
\begin{table}[!t]
\centering
\resizebox{8.3cm}{!}{%
\begin{tabular}{ccccccc}
\Xhline{3\arrayrulewidth}  
\textbf{Sub Func} & \textbf{1} & \textbf{2} & \textbf{4} & \textbf{8} & \textbf{16} & \textbf{Full} \\ \hline
Original     & \textbf{49.58} & 56.83 & 62.70 & 68.41 & 72.49 & 83.97     \\
+ Human     & 48.82 & \textbf{57.10} & \textbf{63.58} & \textbf{69.22} & \textbf{73.24} & \textbf{83.99} \\\Xhline{3\arrayrulewidth}  
\end{tabular}
}
\caption{The performance of LaBo on ImageNet with human intervention. + Human denotes adding the classifier trained on the human-annotated data in the submodular function.}
\end{table}

==> tables/gpt3-regenerate.tex <==
\begin{table}[!t]
\centering
\small
% \resizebox{7.5cm}{!}{%
\begin{tabular}{cccccc}
\Xhline{3\arrayrulewidth}  
\textbf{Concepts} & \textbf{Aircraft} & \textbf{Food} & \textbf{Flower} & \textbf{UCF} & \textbf{CUB }\\ \hline
Original          &   &  &   &   & \\
+ Regenerate      &   &  &   &   &\\\Xhline{3\arrayrulewidth}  
\end{tabular}
% }
\caption{Add the regenerated concepts.}
\end{table}

==> tables/ucf_prompts.tex <==
\begin{table}[!t]
\centering
\small
\begin{tabular}{l}
\Xhline{3\arrayrulewidth}
\multicolumn{1}{c}{\textbf{Prompt Template}}
  \\ \hline
1. describe what the \texttt{[CLASS NAME]} looks like: \\
2. describe the appearance of the \texttt{[CLASS NAME]}: \\
3. describe how to perform the \texttt{[CLASS NAME]}: \\
4. describe a person performing the \texttt{[CLASS NAME]}: \\
5. describe what can you see when a person is \\ ~~~~~performing the \texttt{[CLASS NAME]}: \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{The prompt templates of UCF-101.}
\label{table: ucf prompts}
\end{table}

